Randomness Extraction in AC0 and with Small Locality

Randomness extractors, which extract high quality (almost-uniform) random bits from biased random sources, are important objects both in theory and in practice. While there have been significant progress in obtaining near optimal constructions of randomness extractors in various settings, the computational complexity of randomness extractors is still much less studied. In particular, it is not clear whether randomness extractors with good parameters can be computed in several interesting complexity classes that are much weaker than P. In this paper we study randomness extractors in the following two models of computation: (1) constant-depth circuits (AC0), and (2) the local computation model. Previous work in these models, such as [Vio05a], [GVW15] and [BG13], only achieve constructions with weak parameters. In this work we give explicit constructions of randomness extractors with much better parameters. As an application, we use our AC0 extractors to study pseudorandom generators in AC0, and show that we can construct both cryptographic pseudorandom generators (under reasonable computational assumptions) and unconditional pseudorandom generators for space bounded computation with very good parameters. Our constructions combine several previous techniques in randomness extractors, as well as introduce new techniques to reduce or preserve the complexity of extractors, which may be of independent interest. These include (1) a general way to reduce the error of strong seeded extractors while preserving the AC0 property and small locality, and (2) a seeded randomness condenser with small locality.

==> app.tex <==
For cryptographically secure pseudorandom generators, we mainly adapt the approach of Applebaum \cite{applebaum2013pseudorandom}, to the $\AC^0$ setting. In \cite{applebaum2013pseudorandom}, Applebaum constructed cryptographically secure pseudorandom generator \emph{families} in $\NC^0$. His construction is based on random local functions. Specifically, given a random bipartite graph with $n$ left vertices, $m$ right vertices and right degree $d$ (think of $d$ as a constant), and a suitable predicate $P$ on $d$ bits, Applebaum showed that based on a conjecture on random local one-way functions, the $m$ output bits obtained by applying $P$ to the $m$ subsets of input bits corresponding to the hyper edges give a distribution with high pseudo Shannon entropy. He then showed how to boost the output to have high pseudo min-entropy by concatenating several independent copies. At this point he used an extractor in $\NC^0$ to turn the output into a pseudorandom string. 

However, an extractor in $\NC^0$ needs to have a large seed length (i.e., $\Omega(n)$), thus the $\NC^0$ PRG constructed using this approach only achieves linear stretch. Another issue is that the $\NC^0$ PRG is actually a collection of functions rather than a single function, because the random bits used to sample the bipartite graph is larger than the output length, and is treated as a public index to the collection of functions.

Here, by replacing the extractor with our $\AC^0$ extractor we can achieve a polynomial stretch PRG (based on appropriate assumptions as in \cite{applebaum2013pseudorandom}), although now the PRG is in $\AC^0$ instead of $\NC^0$. In addition, we can get a single PRG instead of a collection of PRG functions, by including the random bits used to sample the bipartite graph as part of the seed. Since in the graph each right vertex only has a constant number $d$ of neighbors, the sampling uses $md \log n$ bits and can be done in $\AC^0$. To ensure that the PRG has a stretch, we take the sampled graph $G$ and apply the \emph{same} graph to several independent copies of $n$ bit input strings. We show that we can still use the method in \cite{applebaum2013pseudorandom} to argue that this gives a a distribution with high pseudo Shannon entropy. We then use the same method as in \cite{applebaum2013pseudorandom} to turn it into a distribution with high pseudo min-entropy, and finally we apply our $\AC^0$ extractor. This way we ensure that the  $md \log n$ bits used to sample the graph $G$ are ``absorbed" by the stretch of the PRG, and thus we get a standard PRG instead of a collection of PRG functions.

For PRGs for space bounded computation, we simply adapt the PRG by Nisan and Zuckerman \cite{NisanZ96}, which stretches $O(S)$ random bits to any $\poly(S)$ bits that fool space $S$ computation. We now replace the seeded extractor used there by our $\AC^0$ extractor. Notice that the Nisan-Zuckerman PRG simply applies the seeded extractor iteratively for a constant number of times, so the whole construction is still in $\AC^0$.
